"Law at Your Fingertips": Understanding Legal Information Seeking on Video-Sharing Platforms in China

Equipping laypeople with the capabilities to seek legal information has been an important goal for Legal Empowerment in modern society. However, unlike general information-seeking behaviors, legal information seeking is characterized by high stakes, urgency, and a critical need for emotional support, which traditional text-based searching platforms struggle to satisfy. In recent years, people have been increasingly turning to Video-Sharing Platforms (VSPs) for access to legal information and to fulfill their legal needs. Despite the importance of this shift, such VSP-mediated legal information-seeking practices remain underexplored. Through an observational analysis of legal content on two VSPs (Douyin and Bilibili) and interviews with 20 Chinese information seekers, this study examined the practices and challenges associated with seeking, comprehending, and evaluating legal information on VSPs. We further revealed the formation of trust and engagement on the VSP-based legal knowledge-sharing community, highlighting how VSP affordances helped mitigate seekers' epistemic discomfort and satisfy their needs for emotional support. In the discussion, we provided insights on balancing heuristic and systematic processing to encourage information cross-validation, and offered implications for designing trustworthy civic information systems and fostering an accessible, safe, and efficient information-seeking environment in digital space.

==> tables/table_short_video.tex <==
\begin{table}[t]
\caption{Presentation Forms of Legal Short Videos}
\resizebox{\textwidth}{!}{\color{blue}\begin{tabular}{|ccl|}
\hline
\textbf{Categories}                                   & \textbf{Presentation Form}                               & \multicolumn{1}{c|}{\textbf{Content}}                                                                                                                                                                             \\ \hline
%\multicolumn{1}{|c|}{\multirow{2}{*}{Live Streaming}} & \multicolumn{1}{c|}{1-on-1 Consultations with Audiences} & \begin{tabular}[c]{@{}l@{}}Influencers allow viewers to phone-in the live streaming \\channel and ask their legal queries.\end{tabular}                                                                \\ \cline{2-3} 
%\multicolumn{1}{|c|}{}                                & \multicolumn{1}{c|}{Answering Questions on Comments}     & \begin{tabular}[c]{@{}l@{}}Similar to 1-on-1 consultations, but instead of viewers \\ phoning-in the live streaming, the influencers will answer\\ questions on the comment section.\end{tabular}                     \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Short Videos}}   & \multicolumn{1}{c|}{Legal Knowledge Explanations}        & \begin{tabular}[c]{@{}l@{}}Typical videos explaining legal knowledge, presented in a \\ variety of different formats, including direct instruction,\\  legal scenarios performing, text description, etc.\end{tabular} \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                & \multicolumn{1}{c|}{Legal Course Recordings}             & \begin{tabular}[c]{@{}l@{}}Video recordings of some legal courses. The presenter is \\ usually a legal scholar or teacher.\end{tabular}                                                                          \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                & \multicolumn{1}{c|}{Live Streaming Recordings}           & \begin{tabular}[c]{@{}l@{}}Replays of legal live streaming for viewers who miss or \\are unable to watch the entire live streaming sessions.\end{tabular}                   \\ \hline
\end{tabular}}
\label{tab: short videos}
\end{table}
